Waverider: Leveraging Hierarchical, Multi-Resolution Maps for Efficient and Reactive Obstacle Avoidance

Fast and reliable obstacle avoidance is an important task for mobile robots. In this work, we propose an efficient reactive system that provides high-quality obstacle avoidance while running at hundreds of hertz with minimal resource usage. Our approach combines wavemap, a hierarchical volumetric map representation, with a novel hierarchical and parallelizable obstacle avoidance algorithm formulated through Riemannian Motion Policies (RMP). Leveraging multi-resolution obstacle avoidance policies, the proposed navigation system facilitates precise, low-latency (36ms), and extremely efficient obstacle avoidance with a very large perceptive radius (30m). We perform extensive statistical evaluations on indoor and outdoor maps, verifying that the proposed system compares favorably to fixed-resolution RMP variants and CHOMP. Finally, the RMP formulation allows the seamless fusion of obstacle avoidance with additional objectives, such as goal-seeking, to obtain a fully-fledged navigation system that is versatile and robust. We deploy the system on a Micro Aerial Vehicle and show how it navigates through an indoor obstacle course. Our complete implementation, called waverider, is made available as open source.

==> abstract.tex <==
waverider: A hierarchical algorithm for efficient, reactive, multi-resolution obstacle avoidance

Reactive, precise, and reliable obstacle avoidance is vital for mobile robots to safely and efficiently navigate our world.
In this work, we propose an efficient reactive system that provides high-quality obstacle avoidance while running at hundreds of hertz with minimal resource usage. 
Our approach combines wavemap, a hierarchical volumetric map representation, with a novel hierarchical and parallelizable obstacle avoidance algorithm formulated through Riemannian Motion Policies (RMP).
Leveraging multi-resolution obstacle avoidance policies, the proposed navigation system facilitates precise, low-latency (35.9ms) obstacle avoidance with a very large perceptive radius (30m) at 200Hz while using only a fraction of the robot's CPU for mapping and planning.
We perform extensive runtime analysis and demonstrate how the proposed algorithm drives a Micro Aerial Vehicle through an obstacle course.
Finally, the RMP formulation makes it possible to seamlessly fuse obstacle avoidance with additional objectives, such as goal-seeking, resulting in a versatile and robust complete navigation system.

Keywords:
Sensing and navigation
Mobile robots
Aerial Robots
